Observation of the $\varXi^{-}_{b}\to J/\psi\varLambda K^{-}$ decay

The observation of the decay $\varXi^{-}_{b}\to J/\psi\varLambda K^{-}$ is reported, using a data sample corresponding to an integrated luminosity of $3~\mathrm{fb}^{-1}$, collected by the LHCb detector in $pp$ collisions at centre-of-mass energies of $7$ and $8~\mathrm{TeV}$. The production rate of $\varXi_{b}^{-}$ baryons detected in the decay $\varXi_{b}^{-}\to J/\psi\varLambda K^{-}$ is measured relative to that of $\varLambda_{b}^{0}$ baryons using the decay $\varLambda_{b}^{0}\to J/\psi \varLambda$. Integrated over the $b$-baryon transverse momentum $p_{\rm T}<25~\mathrm{GeV/}c $ and rapidity $2.0<y<4.5$, the measured ratio is \begin{equation*} \frac{f_{\varXi_{b}^{-}}}{f_{\varLambda_{b}^{0}}}\frac{\mathcal{B}(\varXi_{b}^{-}\to J/\psi\varLambda K^{-})}{\mathcal{B}(\varLambda_{b}^{0}\to J/\psi \varLambda)}=(4.19\pm 0.29~(\mathrm{stat})\pm0.15~(\mathrm{syst}))\times 10^{-2}, \end{equation*}where $f_{\varXi_{b}^{-}}$ and $f_{\varLambda_{b}^{0}}$ are the fragmentation fractions of $b\to\varXi_{b}^{-}$ and $b\to\varLambda_{b}^{0}$ transitions, and $\mathcal{B}$ represents the branching fraction of the corresponding $b$-baryon decay. The mass difference between $\varXi_{b}^{-}$ and $\varLambda_{b}^{0}$ baryons is measured to be \begin{equation*} M(\varXi_{b}^{-})-M(\varLambda_{b}^{0})=177.08\pm0.47~(\mathrm{stat})\pm0.16~(\mathrm{syst} )~\mathrm{MeV/}c^{2}. \end{equation*}

==> LHCb_Authorship_flat_31-Oct-2016.tex <==
\centerline{\large\bf LHCb collaboration}
\begin{flushleft}
\small
R.~Aaij$^{40}$,
B.~Adeva$^{39}$,
M.~Adinolfi$^{48}$,
Z.~Ajaltouni$^{5}$,
S.~Akar$^{59}$,
J.~Albrecht$^{10}$,
F.~Alessio$^{40}$,
M.~Alexander$^{53}$,
S.~Ali$^{43}$,
G.~Alkhazov$^{31}$,
P.~Alvarez~Cartelle$^{55}$,
A.A.~Alves~Jr$^{59}$,
S.~Amato$^{2}$,
S.~Amerio$^{23}$,
Y.~Amhis$^{7}$,
L.~An$^{3}$,
L.~Anderlini$^{18}$,
G.~Andreassi$^{41}$,
M.~Andreotti$^{17,g}$,
J.E.~Andrews$^{60}$,
R.B.~Appleby$^{56}$,
F.~Archilli$^{43}$,
P.~d'Argent$^{12}$,
J.~Arnau~Romeu$^{6}$,
A.~Artamonov$^{37}$,
M.~Artuso$^{61}$,
E.~Aslanides$^{6}$,
G.~Auriemma$^{26}$,
M.~Baalouch$^{5}$,
I.~Babuschkin$^{56}$,
S.~Bachmann$^{12}$,
J.J.~Back$^{50}$,
A.~Badalov$^{38}$,
C.~Baesso$^{62}$,
S.~Baker$^{55}$,
V.~Balagura$^{7,c}$,
W.~Baldini$^{17}$,
R.J.~Barlow$^{56}$,
C.~Barschel$^{40}$,
S.~Barsuk$^{7}$,
W.~Barter$^{40}$,
F.~Baryshnikov$^{32}$,
M.~Baszczyk$^{27}$,
V.~Batozskaya$^{29}$,
B.~Batsukh$^{61}$,
V.~Battista$^{41}$,
A.~Bay$^{41}$,
L.~Beaucourt$^{4}$,
J.~Beddow$^{53}$,
F.~Bedeschi$^{24}$,
I.~Bediaga$^{1}$,
L.J.~Bel$^{43}$,
V.~Bellee$^{41}$,
N.~Belloli$^{21,i}$,
K.~Belous$^{37}$,
I.~Belyaev$^{32}$,
E.~Ben-Haim$^{8}$,
G.~Bencivenni$^{19}$,
S.~Benson$^{43}$,
A.~Berezhnoy$^{33}$,
R.~Bernet$^{42}$,
A.~Bertolin$^{23}$,
C.~Betancourt$^{42}$,
F.~Betti$^{15}$,
M.-O.~Bettler$^{40}$,
M.~van~Beuzekom$^{43}$,
Ia.~Bezshyiko$^{42}$,
S.~Bifani$^{47}$,
P.~Billoir$^{8}$,
T.~Bird$^{56}$,
A.~Birnkraut$^{10}$,
A.~Bitadze$^{56}$,
A.~Bizzeti$^{18,u}$,
T.~Blake$^{50}$,
F.~Blanc$^{41}$,
J.~Blouw$^{11,\dagger}$,
S.~Blusk$^{61}$,
V.~Bocci$^{26}$,
T.~Boettcher$^{58}$,
A.~Bondar$^{36,w}$,
N.~Bondar$^{31,40}$,
W.~Bonivento$^{16}$,
I.~Bordyuzhin$^{32}$,
A.~Borgheresi$^{21,i}$,
S.~Borghi$^{56}$,
M.~Borisyak$^{35}$,
M.~Borsato$^{39}$,
F.~Bossu$^{7}$,
M.~Boubdir$^{9}$,
T.J.V.~Bowcock$^{54}$,
E.~Bowen$^{42}$,
C.~Bozzi$^{17,40}$,
S.~Braun$^{12}$,
M.~Britsch$^{12}$,
T.~Britton$^{61}$,
J.~Brodzicka$^{56}$,
E.~Buchanan$^{48}$,
C.~Burr$^{56}$,
A.~Bursche$^{2}$,
J.~Buytaert$^{40}$,
S.~Cadeddu$^{16}$,
R.~Calabrese$^{17,g}$,
M.~Calvi$^{21,i}$,
M.~Calvo~Gomez$^{38,m}$,
A.~Camboni$^{38}$,
P.~Campana$^{19}$,
D.H.~Campora~Perez$^{40}$,
L.~Capriotti$^{56}$,
A.~Carbone$^{15,e}$,
G.~Carboni$^{25,j}$,
R.~Cardinale$^{20,h}$,
A.~Cardini$^{16}$,
P.~Carniti$^{21,i}$,
L.~Carson$^{52}$,
K.~Carvalho~Akiba$^{2}$,
G.~Casse$^{54}$,
L.~Cassina$^{21,i}$,
L.~Castillo~Garcia$^{41}$,
M.~Cattaneo$^{40}$,
G.~Cavallero$^{20}$,
R.~Cenci$^{24,t}$,
D.~Chamont$^{7}$,
M.~Charles$^{8}$,
Ph.~Charpentier$^{40}$,
G.~Chatzikonstantinidis$^{47}$,
M.~Chefdeville$^{4}$,
S.~Chen$^{56}$,
S.-F.~Cheung$^{57}$,
V.~Chobanova$^{39}$,
M.~Chrzaszcz$^{42,27}$,
X.~Cid~Vidal$^{39}$,
G.~Ciezarek$^{43}$,
P.E.L.~Clarke$^{52}$,
M.~Clemencic$^{40}$,
H.V.~Cliff$^{49}$,
J.~Closier$^{40}$,
V.~Coco$^{59}$,
J.~Cogan$^{6}$,
E.~Cogneras$^{5}$,
V.~Cogoni$^{16,40,f}$,
L.~Cojocariu$^{30}$,
G.~Collazuol$^{23,o}$,
P.~Collins$^{40}$,
A.~Comerma-Montells$^{12}$,
A.~Contu$^{40}$,
A.~Cook$^{48}$,
G.~Coombs$^{40}$,
S.~Coquereau$^{38}$,
G.~Corti$^{40}$,
M.~Corvo$^{17,g}$,
C.M.~Costa~Sobral$^{50}$,
B.~Couturier$^{40}$,
G.A.~Cowan$^{52}$,
D.C.~Craik$^{52}$,
A.~Crocombe$^{50}$,
M.~Cruz~Torres$^{62}$,
S.~Cunliffe$^{55}$,
R.~Currie$^{55}$,
C.~D'Ambrosio$^{40}$,
F.~Da~Cunha~Marinho$^{2}$,
E.~Dall'Occo$^{43}$,
J.~Dalseno$^{48}$,
P.N.Y.~David$^{43}$,
A.~Davis$^{3}$,
K.~De~Bruyn$^{6}$,
S.~De~Capua$^{56}$,
M.~De~Cian$^{12}$,
J.M.~De~Miranda$^{1}$,
L.~De~Paula$^{2}$,
M.~De~Serio$^{14,d}$,
P.~De~Simone$^{19}$,
C.T.~Dean$^{53}$,
D.~Decamp$^{4}$,
M.~Deckenhoff$^{10}$,
L.~Del~Buono$^{8}$,
M.~Demmer$^{10}$,
A.~Dendek$^{28}$,
D.~Derkach$^{35}$,
O.~Deschamps$^{5}$,
F.~Dettori$^{40}$,
B.~Dey$^{22}$,
A.~Di~Canto$^{40}$,
H.~Dijkstra$^{40}$,
F.~Dordei$^{40}$,
M.~Dorigo$^{41}$,
A.~Dosil~Su{\'a}rez$^{39}$,
A.~Dovbnya$^{45}$,
K.~Dreimanis$^{54}$,
L.~Dufour$^{43}$,
G.~Dujany$^{56}$,
K.~Dungs$^{40}$,
P.~Durante$^{40}$,
R.~Dzhelyadin$^{37}$,
A.~Dziurda$^{40}$,
A.~Dzyuba$^{31}$,
N.~D{\'e}l{\'e}age$^{4}$,
S.~Easo$^{51}$,
M.~Ebert$^{52}$,
U.~Egede$^{55}$,
V.~Egorychev$^{32}$,
S.~Eidelman$^{36,w}$,
S.~Eisenhardt$^{52}$,
U.~Eitschberger$^{10}$,
R.~Ekelhof$^{10}$,
L.~Eklund$^{53}$,
S.~Ely$^{61}$,
S.~Esen$^{12}$,
H.M.~Evans$^{49}$,
T.~Evans$^{57}$,
A.~Falabella$^{15}$,
N.~Farley$^{47}$,
S.~Farry$^{54}$,
R.~Fay$^{54}$,
D.~Fazzini$^{21,i}$,
D.~Ferguson$^{52}$,
A.~Fernandez~Prieto$^{39}$,
F.~Ferrari$^{15,40}$,
F.~Ferreira~Rodrigues$^{2}$,
M.~Ferro-Luzzi$^{40}$,
S.~Filippov$^{34}$,
R.A.~Fini$^{14}$,
M.~Fiore$^{17,g}$,
M.~Fiorini$^{17,g}$,
M.~Firlej$^{28}$,
C.~Fitzpatrick$^{41}$,
T.~Fiutowski$^{28}$,
F.~Fleuret$^{7,b}$,
K.~Fohl$^{40}$,
M.~Fontana$^{16,40}$,
F.~Fontanelli$^{20,h}$,
D.C.~Forshaw$^{61}$,
R.~Forty$^{40}$,
V.~Franco~Lima$^{54}$,
M.~Frank$^{40}$,
C.~Frei$^{40}$,
J.~Fu$^{22,q}$,
W.~Funk$^{40}$,
E.~Furfaro$^{25,j}$,
C.~F{\"a}rber$^{40}$,
A.~Gallas~Torreira$^{39}$,
D.~Galli$^{15,e}$,
S.~Gallorini$^{23}$,
S.~Gambetta$^{52}$,
M.~Gandelman$^{2}$,
P.~Gandini$^{57}$,
Y.~Gao$^{3}$,
L.M.~Garcia~Martin$^{69}$,
J.~Garc{\'\i}a~Pardi{\~n}as$^{39}$,
J.~Garra~Tico$^{49}$,
L.~Garrido$^{38}$,
P.J.~Garsed$^{49}$,
D.~Gascon$^{38}$,
C.~Gaspar$^{40}$,
L.~Gavardi$^{10}$,
G.~Gazzoni$^{5}$,
D.~Gerick$^{12}$,
E.~Gersabeck$^{12}$,
M.~Gersabeck$^{56}$,
T.~Gershon$^{50}$,
Ph.~Ghez$^{4}$,
S.~Gian{\`\i}$^{41}$,
V.~Gibson$^{49}$,
O.G.~Girard$^{41}$,
L.~Giubega$^{30}$,
K.~Gizdov$^{52}$,
V.V.~Gligorov$^{8}$,
D.~Golubkov$^{32}$,
A.~Golutvin$^{55,40}$,
A.~Gomes$^{1,a}$,
I.V.~Gorelov$^{33}$,
C.~Gotti$^{21,i}$,
R.~Graciani~Diaz$^{38}$,
L.A.~Granado~Cardoso$^{40}$,
E.~Graug{\'e}s$^{38}$,
E.~Graverini$^{42}$,
G.~Graziani$^{18}$,
A.~Grecu$^{30}$,
P.~Griffith$^{47}$,
L.~Grillo$^{21,40,i}$,
B.R.~Gruberg~Cazon$^{57}$,
O.~Gr{\"u}nberg$^{67}$,
E.~Gushchin$^{34}$,
Yu.~Guz$^{37}$,
T.~Gys$^{40}$,
C.~G{\"o}bel$^{62}$,
T.~Hadavizadeh$^{57}$,
C.~Hadjivasiliou$^{5}$,
G.~Haefeli$^{41}$,
C.~Haen$^{40}$,
S.C.~Haines$^{49}$,
B.~Hamilton$^{60}$,
X.~Han$^{12}$,
S.~Hansmann-Menzemer$^{12}$,
N.~Harnew$^{57}$,
S.T.~Harnew$^{48}$,
J.~Harrison$^{56}$,
M.~Hatch$^{40}$,
J.~He$^{63}$,
T.~Head$^{41}$,
A.~Heister$^{9}$,
K.~Hennessy$^{54}$,
P.~Henrard$^{5}$,
L.~Henry$^{8}$,
E.~van~Herwijnen$^{40}$,
M.~He{\ss}$^{67}$,
A.~Hicheur$^{2}$,
D.~Hill$^{57}$,
C.~Hombach$^{56}$,
H.~Hopchev$^{41}$,
W.~Hulsbergen$^{43}$,
T.~Humair$^{55}$,
M.~Hushchyn$^{35}$,
D.~Hutchcroft$^{54}$,
M.~Idzik$^{28}$,
P.~Ilten$^{58}$,
R.~Jacobsson$^{40}$,
A.~Jaeger$^{12}$,
J.~Jalocha$^{57}$,
E.~Jans$^{43}$,
A.~Jawahery$^{60}$,
F.~Jiang$^{3}$,
M.~John$^{57}$,
D.~Johnson$^{40}$,
C.R.~Jones$^{49}$,
C.~Joram$^{40}$,
B.~Jost$^{40}$,
N.~Jurik$^{57}$,
S.~Kandybei$^{45}$,
M.~Karacson$^{40}$,
J.M.~Kariuki$^{48}$,
S.~Karodia$^{53}$,
M.~Kecke$^{12}$,
M.~Kelsey$^{61}$,
M.~Kenzie$^{49}$,
T.~Ketel$^{44}$,
E.~Khairullin$^{35}$,
B.~Khanji$^{12}$,
C.~Khurewathanakul$^{41}$,
T.~Kirn$^{9}$,
S.~Klaver$^{56}$,
K.~Klimaszewski$^{29}$,
S.~Koliiev$^{46}$,
M.~Kolpin$^{12}$,
I.~Komarov$^{41}$,
R.F.~Koopman$^{44}$,
P.~Koppenburg$^{43}$,
A.~Kosmyntseva$^{32}$,
A.~Kozachuk$^{33}$,
M.~Kozeiha$^{5}$,
L.~Kravchuk$^{34}$,
K.~Kreplin$^{12}$,
M.~Kreps$^{50}$,
P.~Krokovny$^{36,w}$,
F.~Kruse$^{10}$,
W.~Krzemien$^{29}$,
W.~Kucewicz$^{27,l}$,
M.~Kucharczyk$^{27}$,
V.~Kudryavtsev$^{36,w}$,
A.K.~Kuonen$^{41}$,
K.~Kurek$^{29}$,
T.~Kvaratskheliya$^{32,40}$,
D.~Lacarrere$^{40}$,
G.~Lafferty$^{56}$,
A.~Lai$^{16}$,
G.~Lanfranchi$^{19}$,
C.~Langenbruch$^{9}$,
T.~Latham$^{50}$,
C.~Lazzeroni$^{47}$,
R.~Le~Gac$^{6}$,
J.~van~Leerdam$^{43}$,
A.~Leflat$^{33,40}$,
J.~Lefran{\c{c}}ois$^{7}$,
R.~Lef{\`e}vre$^{5}$,
F.~Lemaitre$^{40}$,
E.~Lemos~Cid$^{39}$,
O.~Leroy$^{6}$,
T.~Lesiak$^{27}$,
B.~Leverington$^{12}$,
T.~Li$^{3}$,
Y.~Li$^{7}$,
T.~Likhomanenko$^{35,68}$,
R.~Lindner$^{40}$,
C.~Linn$^{40}$,
F.~Lionetto$^{42}$,
X.~Liu$^{3}$,
D.~Loh$^{50}$,
I.~Longstaff$^{53}$,
J.H.~Lopes$^{2}$,
D.~Lucchesi$^{23,o}$,
M.~Lucio~Martinez$^{39}$,
H.~Luo$^{52}$,
A.~Lupato$^{23}$,
E.~Luppi$^{17,g}$,
O.~Lupton$^{40}$,
A.~Lusiani$^{24}$,
X.~Lyu$^{63}$,
F.~Machefert$^{7}$,
F.~Maciuc$^{30}$,
O.~Maev$^{31}$,
K.~Maguire$^{56}$,
S.~Malde$^{57}$,
A.~Malinin$^{68}$,
T.~Maltsev$^{36}$,
G.~Manca$^{16,f}$,
G.~Mancinelli$^{6}$,
P.~Manning$^{61}$,
J.~Maratas$^{5,v}$,
J.F.~Marchand$^{4}$,
U.~Marconi$^{15}$,
C.~Marin~Benito$^{38}$,
M.~Marinangeli$^{41}$,
P.~Marino$^{24,t}$,
J.~Marks$^{12}$,
G.~Martellotti$^{26}$,
M.~Martin$^{6}$,
M.~Martinelli$^{41}$,
D.~Martinez~Santos$^{39}$,
F.~Martinez~Vidal$^{69}$,
D.~Martins~Tostes$^{2}$,
L.M.~Massacrier$^{7}$,
A.~Massafferri$^{1}$,
R.~Matev$^{40}$,
A.~Mathad$^{50}$,
Z.~Mathe$^{40}$,
C.~Matteuzzi$^{21}$,
A.~Mauri$^{42}$,
E.~Maurice$^{7,b}$,
B.~Maurin$^{41}$,
A.~Mazurov$^{47}$,
M.~McCann$^{55,40}$,
A.~McNab$^{56}$,
R.~McNulty$^{13}$,
B.~Meadows$^{59}$,
F.~Meier$^{10}$,
M.~Meissner$^{12}$,
D.~Melnychuk$^{29}$,
M.~Merk$^{43}$,
A.~Merli$^{22,q}$,
E.~Michielin$^{23}$,
D.A.~Milanes$^{66}$,
M.-N.~Minard$^{4}$,
D.S.~Mitzel$^{12}$,
A.~Mogini$^{8}$,
J.~Molina~Rodriguez$^{1}$,
I.A.~Monroy$^{66}$,
S.~Monteil$^{5}$,
M.~Morandin$^{23}$,
P.~Morawski$^{28}$,
A.~Mord{\`a}$^{6}$,
M.J.~Morello$^{24,t}$,
O.~Morgunova$^{68}$,
J.~Moron$^{28}$,
A.B.~Morris$^{52}$,
R.~Mountain$^{61}$,
F.~Muheim$^{52}$,
M.~Mulder$^{43}$,
M.~Mussini$^{15}$,
D.~M{\"u}ller$^{56}$,
J.~M{\"u}ller$^{10}$,
K.~M{\"u}ller$^{42}$,
V.~M{\"u}ller$^{10}$,
P.~Naik$^{48}$,
T.~Nakada$^{41}$,
R.~Nandakumar$^{51}$,
A.~Nandi$^{57}$,
I.~Nasteva$^{2}$,
M.~Needham$^{52}$,
N.~Neri$^{22}$,
S.~Neubert$^{12}$,
N.~Neufeld$^{40}$,
M.~Neuner$^{12}$,
T.D.~Nguyen$^{41}$,
C.~Nguyen-Mau$^{41,n}$,
S.~Nieswand$^{9}$,
R.~Niet$^{10}$,
N.~Nikitin$^{33}$,
T.~Nikodem$^{12}$,
A.~Nogay$^{68}$,
A.~Novoselov$^{37}$,
D.P.~O'Hanlon$^{50}$,
A.~Oblakowska-Mucha$^{28}$,
V.~Obraztsov$^{37}$,
S.~Ogilvy$^{19}$,
R.~Oldeman$^{16,f}$,
C.J.G.~Onderwater$^{70}$,
J.M.~Otalora~Goicochea$^{2}$,
A.~Otto$^{40}$,
P.~Owen$^{42}$,
A.~Oyanguren$^{69}$,
P.R.~Pais$^{41}$,
A.~Palano$^{14,d}$,
F.~Palombo$^{22,q}$,
M.~Palutan$^{19}$,
A.~Papanestis$^{51}$,
M.~Pappagallo$^{14,d}$,
L.L.~Pappalardo$^{17,g}$,
W.~Parker$^{60}$,
C.~Parkes$^{56}$,
G.~Passaleva$^{18}$,
A.~Pastore$^{14,d}$,
G.D.~Patel$^{54}$,
M.~Patel$^{55}$,
C.~Patrignani$^{15,e}$,
A.~Pearce$^{40}$,
A.~Pellegrino$^{43}$,
G.~Penso$^{26}$,
M.~Pepe~Altarelli$^{40}$,
S.~Perazzini$^{40}$,
P.~Perret$^{5}$,
L.~Pescatore$^{47}$,
K.~Petridis$^{48}$,
A.~Petrolini$^{20,h}$,
A.~Petrov$^{68}$,
M.~Petruzzo$^{22,q}$,
E.~Picatoste~Olloqui$^{38}$,
B.~Pietrzyk$^{4}$,
M.~Pikies$^{27}$,
D.~Pinci$^{26}$,
A.~Pistone$^{20}$,
A.~Piucci$^{12}$,
V.~Placinta$^{30}$,
S.~Playfer$^{52}$,
M.~Plo~Casasus$^{39}$,
T.~Poikela$^{40}$,
F.~Polci$^{8}$,
A.~Poluektov$^{50,36}$,
I.~Polyakov$^{61}$,
E.~Polycarpo$^{2}$,
G.J.~Pomery$^{48}$,
A.~Popov$^{37}$,
D.~Popov$^{11,40}$,
B.~Popovici$^{30}$,
S.~Poslavskii$^{37}$,
C.~Potterat$^{2}$,
E.~Price$^{48}$,
J.D.~Price$^{54}$,
J.~Prisciandaro$^{39,40}$,
A.~Pritchard$^{54}$,
C.~Prouve$^{48}$,
V.~Pugatch$^{46}$,
A.~Puig~Navarro$^{42}$,
G.~Punzi$^{24,p}$,
W.~Qian$^{50}$,
R.~Quagliani$^{7,48}$,
B.~Rachwal$^{27}$,
J.H.~Rademacker$^{48}$,
M.~Rama$^{24}$,
M.~Ramos~Pernas$^{39}$,
M.S.~Rangel$^{2}$,
I.~Raniuk$^{45}$,
F.~Ratnikov$^{35}$,
G.~Raven$^{44}$,
F.~Redi$^{55}$,
S.~Reichert$^{10}$,
A.C.~dos~Reis$^{1}$,
C.~Remon~Alepuz$^{69}$,
V.~Renaudin$^{7}$,
S.~Ricciardi$^{51}$,
S.~Richards$^{48}$,
M.~Rihl$^{40}$,
K.~Rinnert$^{54}$,
V.~Rives~Molina$^{38}$,
P.~Robbe$^{7,40}$,
A.B.~Rodrigues$^{1}$,
E.~Rodrigues$^{59}$,
J.A.~Rodriguez~Lopez$^{66}$,
P.~Rodriguez~Perez$^{56,\dagger}$,
A.~Rogozhnikov$^{35}$,
S.~Roiser$^{40}$,
A.~Rollings$^{57}$,
V.~Romanovskiy$^{37}$,
A.~Romero~Vidal$^{39}$,
J.W.~Ronayne$^{13}$,
M.~Rotondo$^{19}$,
M.S.~Rudolph$^{61}$,
T.~Ruf$^{40}$,
P.~Ruiz~Valls$^{69}$,
J.J.~Saborido~Silva$^{39}$,
E.~Sadykhov$^{32}$,
N.~Sagidova$^{31}$,
B.~Saitta$^{16,f}$,
V.~Salustino~Guimaraes$^{1}$,
C.~Sanchez~Mayordomo$^{69}$,
B.~Sanmartin~Sedes$^{39}$,
R.~Santacesaria$^{26}$,
C.~Santamarina~Rios$^{39}$,
M.~Santimaria$^{19}$,
E.~Santovetti$^{25,j}$,
A.~Sarti$^{19,k}$,
C.~Satriano$^{26,s}$,
A.~Satta$^{25}$,
D.M.~Saunders$^{48}$,
D.~Savrina$^{32,33}$,
S.~Schael$^{9}$,
M.~Schellenberg$^{10}$,
M.~Schiller$^{53}$,
H.~Schindler$^{40}$,
M.~Schlupp$^{10}$,
M.~Schmelling$^{11}$,
T.~Schmelzer$^{10}$,
B.~Schmidt$^{40}$,
O.~Schneider$^{41}$,
A.~Schopper$^{40}$,
K.~Schubert$^{10}$,
M.~Schubiger$^{41}$,
M.-H.~Schune$^{7}$,
R.~Schwemmer$^{40}$,
B.~Sciascia$^{19}$,
A.~Sciubba$^{26,k}$,
A.~Semennikov$^{32}$,
A.~Sergi$^{47}$,
N.~Serra$^{42}$,
J.~Serrano$^{6}$,
L.~Sestini$^{23}$,
P.~Seyfert$^{21}$,
M.~Shapkin$^{37}$,
I.~Shapoval$^{45}$,
Y.~Shcheglov$^{31}$,
T.~Shears$^{54}$,
L.~Shekhtman$^{36,w}$,
V.~Shevchenko$^{68}$,
B.G.~Siddi$^{17,40}$,
R.~Silva~Coutinho$^{42}$,
L.~Silva~de~Oliveira$^{2}$,
G.~Simi$^{23,o}$,
S.~Simone$^{14,d}$,
M.~Sirendi$^{49}$,
N.~Skidmore$^{48}$,
T.~Skwarnicki$^{61}$,
E.~Smith$^{55}$,
I.T.~Smith$^{52}$,
J.~Smith$^{49}$,
M.~Smith$^{55}$,
H.~Snoek$^{43}$,
l.~Soares~Lavra$^{1}$,
M.D.~Sokoloff$^{59}$,
F.J.P.~Soler$^{53}$,
B.~Souza~De~Paula$^{2}$,
B.~Spaan$^{10}$,
P.~Spradlin$^{53}$,
S.~Sridharan$^{40}$,
F.~Stagni$^{40}$,
M.~Stahl$^{12}$,
S.~Stahl$^{40}$,
P.~Stefko$^{41}$,
S.~Stefkova$^{55}$,
O.~Steinkamp$^{42}$,
S.~Stemmle$^{12}$,
O.~Stenyakin$^{37}$,
H.~Stevens$^{10}$,
S.~Stevenson$^{57}$,
S.~Stoica$^{30}$,
S.~Stone$^{61}$,
B.~Storaci$^{42}$,
S.~Stracka$^{24,p}$,
M.~Straticiuc$^{30}$,
U.~Straumann$^{42}$,
L.~Sun$^{64}$,
W.~Sutcliffe$^{55}$,
K.~Swientek$^{28}$,
V.~Syropoulos$^{44}$,
M.~Szczekowski$^{29}$,
T.~Szumlak$^{28}$,
S.~T'Jampens$^{4}$,
A.~Tayduganov$^{6}$,
T.~Tekampe$^{10}$,
G.~Tellarini$^{17,g}$,
F.~Teubert$^{40}$,
E.~Thomas$^{40}$,
J.~van~Tilburg$^{43}$,
M.J.~Tilley$^{55}$,
V.~Tisserand$^{4}$,
M.~Tobin$^{41}$,
S.~Tolk$^{49}$,
L.~Tomassetti$^{17,g}$,
D.~Tonelli$^{40}$,
S.~Topp-Joergensen$^{57}$,
F.~Toriello$^{61}$,
E.~Tournefier$^{4}$,
S.~Tourneur$^{41}$,
K.~Trabelsi$^{41}$,
M.~Traill$^{53}$,
M.T.~Tran$^{41}$,
M.~Tresch$^{42}$,
A.~Trisovic$^{40}$,
A.~Tsaregorodtsev$^{6}$,
P.~Tsopelas$^{43}$,
A.~Tully$^{49}$,
N.~Tuning$^{43}$,
A.~Ukleja$^{29}$,
A.~Ustyuzhanin$^{35}$,
U.~Uwer$^{12}$,
C.~Vacca$^{16,f}$,
V.~Vagnoni$^{15,40}$,
A.~Valassi$^{40}$,
S.~Valat$^{40}$,
G.~Valenti$^{15}$,
R.~Vazquez~Gomez$^{19}$,
P.~Vazquez~Regueiro$^{39}$,
S.~Vecchi$^{17}$,
M.~van~Veghel$^{43}$,
J.J.~Velthuis$^{48}$,
M.~Veltri$^{18,r}$,
G.~Veneziano$^{57}$,
A.~Venkateswaran$^{61}$,
M.~Vernet$^{5}$,
M.~Vesterinen$^{12}$,
J.V.~Viana~Barbosa$^{40}$,
B.~Viaud$^{7}$,
D.~~Vieira$^{63}$,
M.~Vieites~Diaz$^{39}$,
H.~Viemann$^{67}$,
X.~Vilasis-Cardona$^{38,m}$,
M.~Vitti$^{49}$,
V.~Volkov$^{33}$,
A.~Vollhardt$^{42}$,
B.~Voneki$^{40}$,
A.~Vorobyev$^{31}$,
V.~Vorobyev$^{36,w}$,
C.~Vo{\ss}$^{9}$,
J.A.~de~Vries$^{43}$,
C.~V{\'a}zquez~Sierra$^{39}$,
R.~Waldi$^{67}$,
C.~Wallace$^{50}$,
R.~Wallace$^{13}$,
J.~Walsh$^{24}$,
J.~Wang$^{61}$,
D.R.~Ward$^{49}$,
H.M.~Wark$^{54}$,
N.K.~Watson$^{47}$,
D.~Websdale$^{55}$,
A.~Weiden$^{42}$,
M.~Whitehead$^{40}$,
J.~Wicht$^{50}$,
G.~Wilkinson$^{57,40}$,
M.~Wilkinson$^{61}$,
M.~Williams$^{40}$,
M.P.~Williams$^{47}$,
M.~Williams$^{58}$,
T.~Williams$^{47}$,
F.F.~Wilson$^{51}$,
J.~Wimberley$^{60}$,
J.~Wishahi$^{10}$,
W.~Wislicki$^{29}$,
M.~Witek$^{27}$,
G.~Wormser$^{7}$,
S.A.~Wotton$^{49}$,
K.~Wraight$^{53}$,
K.~Wyllie$^{40}$,
Y.~Xie$^{65}$,
Z.~Xing$^{61}$,
Z.~Xu$^{41}$,
Z.~Yang$^{3}$,
Y.~Yao$^{61}$,
H.~Yin$^{65}$,
J.~Yu$^{65}$,
X.~Yuan$^{36,w}$,
O.~Yushchenko$^{37}$,
K.A.~Zarebski$^{47}$,
M.~Zavertyaev$^{11,c}$,
L.~Zhang$^{3}$,
Y.~Zhang$^{7}$,
Y.~Zhang$^{63}$,
A.~Zhelezov$^{12}$,
Y.~Zheng$^{63}$,
X.~Zhu$^{3}$,
V.~Zhukov$^{33}$,
S.~Zucchelli$^{15}$.\bigskip

{\footnotesize \it
$ ^{1}$Centro Brasileiro de Pesquisas F{\'\i}sicas (CBPF), Rio de Janeiro, Brazil\\
$ ^{2}$Universidade Federal do Rio de Janeiro (UFRJ), Rio de Janeiro, Brazil\\
$ ^{3}$Center for High Energy Physics, Tsinghua University, Beijing, China\\
$ ^{4}$LAPP, Universit{\'e} Savoie Mont-Blanc, CNRS/IN2P3, Annecy-Le-Vieux, France\\
$ ^{5}$Clermont Universit{\'e}, Universit{\'e} Blaise Pascal, CNRS/IN2P3, LPC, Clermont-Ferrand, France\\
$ ^{6}$CPPM, Aix-Marseille Universit{\'e}, CNRS/IN2P3, Marseille, France\\
$ ^{7}$LAL, Universit{\'e} Paris-Sud, CNRS/IN2P3, Orsay, France\\
$ ^{8}$LPNHE, Universit{\'e} Pierre et Marie Curie, Universit{\'e} Paris Diderot, CNRS/IN2P3, Paris, France\\
$ ^{9}$I. Physikalisches Institut, RWTH Aachen University, Aachen, Germany\\
$ ^{10}$Fakult{\"a}t Physik, Technische Universit{\"a}t Dortmund, Dortmund, Germany\\
$ ^{11}$Max-Planck-Institut f{\"u}r Kernphysik (MPIK), Heidelberg, Germany\\
$ ^{12}$Physikalisches Institut, Ruprecht-Karls-Universit{\"a}t Heidelberg, Heidelberg, Germany\\
$ ^{13}$School of Physics, University College Dublin, Dublin, Ireland\\
$ ^{14}$Sezione INFN di Bari, Bari, Italy\\
$ ^{15}$Sezione INFN di Bologna, Bologna, Italy\\
$ ^{16}$Sezione INFN di Cagliari, Cagliari, Italy\\
$ ^{17}$Sezione INFN di Ferrara, Ferrara, Italy\\
$ ^{18}$Sezione INFN di Firenze, Firenze, Italy\\
$ ^{19}$Laboratori Nazionali dell'INFN di Frascati, Frascati, Italy\\
$ ^{20}$Sezione INFN di Genova, Genova, Italy\\
$ ^{21}$Sezione INFN di Milano Bicocca, Milano, Italy\\
$ ^{22}$Sezione INFN di Milano, Milano, Italy\\
$ ^{23}$Sezione INFN di Padova, Padova, Italy\\
$ ^{24}$Sezione INFN di Pisa, Pisa, Italy\\
$ ^{25}$Sezione INFN di Roma Tor Vergata, Roma, Italy\\
$ ^{26}$Sezione INFN di Roma La Sapienza, Roma, Italy\\
$ ^{27}$Henryk Niewodniczanski Institute of Nuclear Physics  Polish Academy of Sciences, Krak{\'o}w, Poland\\
$ ^{28}$AGH - University of Science and Technology, Faculty of Physics and Applied Computer Science, Krak{\'o}w, Poland\\
$ ^{29}$National Center for Nuclear Research (NCBJ), Warsaw, Poland\\
$ ^{30}$Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest-Magurele, Romania\\
$ ^{31}$Petersburg Nuclear Physics Institute (PNPI), Gatchina, Russia\\
$ ^{32}$Institute of Theoretical and Experimental Physics (ITEP), Moscow, Russia\\
$ ^{33}$Institute of Nuclear Physics, Moscow State University (SINP MSU), Moscow, Russia\\
$ ^{34}$Institute for Nuclear Research of the Russian Academy of Sciences (INR RAN), Moscow, Russia\\
$ ^{35}$Yandex School of Data Analysis, Moscow, Russia\\
$ ^{36}$Budker Institute of Nuclear Physics (SB RAS), Novosibirsk, Russia\\
$ ^{37}$Institute for High Energy Physics (IHEP), Protvino, Russia\\
$ ^{38}$ICCUB, Universitat de Barcelona, Barcelona, Spain\\
$ ^{39}$Universidad de Santiago de Compostela, Santiago de Compostela, Spain\\
$ ^{40}$European Organization for Nuclear Research (CERN), Geneva, Switzerland\\
$ ^{41}$Institute of Physics, Ecole Polytechnique  F{\'e}d{\'e}rale de Lausanne (EPFL), Lausanne, Switzerland\\
$ ^{42}$Physik-Institut, Universit{\"a}t Z{\"u}rich, Z{\"u}rich, Switzerland\\
$ ^{43}$Nikhef National Institute for Subatomic Physics, Amsterdam, The Netherlands\\
$ ^{44}$Nikhef National Institute for Subatomic Physics and VU University Amsterdam, Amsterdam, The Netherlands\\
$ ^{45}$NSC Kharkiv Institute of Physics and Technology (NSC KIPT), Kharkiv, Ukraine\\
$ ^{46}$Institute for Nuclear Research of the National Academy of Sciences (KINR), Kyiv, Ukraine\\
$ ^{47}$University of Birmingham, Birmingham, United Kingdom\\
$ ^{48}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom\\
$ ^{49}$Cavendish Laboratory, University of Cambridge, Cambridge, United Kingdom\\
$ ^{50}$Department of Physics, University of Warwick, Coventry, United Kingdom\\
$ ^{51}$STFC Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$ ^{52}$School of Physics and Astronomy, University of Edinburgh, Edinburgh, United Kingdom\\
$ ^{53}$School of Physics and Astronomy, University of Glasgow, Glasgow, United Kingdom\\
$ ^{54}$Oliver Lodge Laboratory, University of Liverpool, Liverpool, United Kingdom\\
$ ^{55}$Imperial College London, London, United Kingdom\\
$ ^{56}$School of Physics and Astronomy, University of Manchester, Manchester, United Kingdom\\
$ ^{57}$Department of Physics, University of Oxford, Oxford, United Kingdom\\
$ ^{58}$Massachusetts Institute of Technology, Cambridge, MA, United States\\
$ ^{59}$University of Cincinnati, Cincinnati, OH, United States\\
$ ^{60}$University of Maryland, College Park, MD, United States\\
$ ^{61}$Syracuse University, Syracuse, NY, United States\\
$ ^{62}$Pontif{\'\i}cia Universidade Cat{\'o}lica do Rio de Janeiro (PUC-Rio), Rio de Janeiro, Brazil, associated to $^{2}$\\
$ ^{63}$University of Chinese Academy of Sciences, Beijing, China, associated to $^{3}$\\
$ ^{64}$School of Physics and Technology, Wuhan University, Wuhan, China, associated to $^{3}$\\
$ ^{65}$Institute of Particle Physics, Central China Normal University, Wuhan, Hubei, China, associated to $^{3}$\\
$ ^{66}$Departamento de Fisica , Universidad Nacional de Colombia, Bogota, Colombia, associated to $^{8}$\\
$ ^{67}$Institut f{\"u}r Physik, Universit{\"a}t Rostock, Rostock, Germany, associated to $^{12}$\\
$ ^{68}$National Research Centre Kurchatov Institute, Moscow, Russia, associated to $^{32}$\\
$ ^{69}$Instituto de Fisica Corpuscular, Centro Mixto Universidad de Valencia - CSIC, Valencia, Spain, associated to $^{38}$\\
$ ^{70}$Van Swinderen Institute, University of Groningen, Groningen, The Netherlands, associated to $^{43}$\\
\bigskip
$ ^{a}$Universidade Federal do Tri{\^a}ngulo Mineiro (UFTM), Uberaba-MG, Brazil\\
$ ^{b}$Laboratoire Leprince-Ringuet, Palaiseau, France\\
$ ^{c}$P.N. Lebedev Physical Institute, Russian Academy of Science (LPI RAS), Moscow, Russia\\
$ ^{d}$Universit{\`a} di Bari, Bari, Italy\\
$ ^{e}$Universit{\`a} di Bologna, Bologna, Italy\\
$ ^{f}$Universit{\`a} di Cagliari, Cagliari, Italy\\
$ ^{g}$Universit{\`a} di Ferrara, Ferrara, Italy\\
$ ^{h}$Universit{\`a} di Genova, Genova, Italy\\
$ ^{i}$Universit{\`a} di Milano Bicocca, Milano, Italy\\
$ ^{j}$Universit{\`a} di Roma Tor Vergata, Roma, Italy\\
$ ^{k}$Universit{\`a} di Roma La Sapienza, Roma, Italy\\
$ ^{l}$AGH - University of Science and Technology, Faculty of Computer Science, Electronics and Telecommunications, Krak{\'o}w, Poland\\
$ ^{m}$LIFAELS, La Salle, Universitat Ramon Llull, Barcelona, Spain\\
$ ^{n}$Hanoi University of Science, Hanoi, Viet Nam\\
$ ^{o}$Universit{\`a} di Padova, Padova, Italy\\
$ ^{p}$Universit{\`a} di Pisa, Pisa, Italy\\
$ ^{q}$Universit{\`a} degli Studi di Milano, Milano, Italy\\
$ ^{r}$Universit{\`a} di Urbino, Urbino, Italy\\
$ ^{s}$Universit{\`a} della Basilicata, Potenza, Italy\\
$ ^{t}$Scuola Normale Superiore, Pisa, Italy\\
$ ^{u}$Universit{\`a} di Modena e Reggio Emilia, Modena, Italy\\
$ ^{v}$Iligan Institute of Technology (IIT), Iligan, Philippines\\
$ ^{w}$Novosibirsk State University, Novosibirsk, Russia\\
\medskip
$ ^{\dagger}$Deceased
}
\end{flushleft}
